Conformance Checking with Uncertainty via SMT (Extended Version)

Logs of real-life processes often feature uncertainty pertaining the recorded timestamps, data values, and/or events. We consider the problem of checking conformance of uncertain logs against data-aware reference processes. Specifically, we show how to solve it via SMT encodings, lifting previous work on data-aware SMT-based conformance checking to this more sophisticated setting. Our approach is modular, in that it homogeneously accommodates for different types of uncertainty. Moreover, using appropriate cost functions, different conformance checking tasks can be addressed. We show the correctness of our approach and witness feasibility through a proof-of-concept implementation.

==> 3-uncertainty.tex <==
%!TEX root = main.tex

Process mining is a well-established field of research at the intersection between BPM and data science. The vast majority of process mining tasks assumes that their input event data provide an accurate and complete digital footprint of reality \cite{Aals11}. In many settings, this is an unrealistic assumption: events may be missing or totally/partially wrongly recorded, due to various factors such as human errors, faulty loggers, errors in the acquisition of events (e.g., through sensors), etc. To mitigate this issue, two lines of research emerged lately. The first deals with methodologies and techniques to improve the quality of event data, thus handling uncertainty in the data preparation phase \cite{WynS19}. The second instead aims at incorporating the management of uncertainty within the process mining tasks themselves, leading to a new generation of process mining techniques where process models \cite{LABP21,PolK22,BMMP21,AMMP22} and/or event logs \cite{PegoraroUA21,CMMF18} explicitly address different kinds of uncertainty. 

Surprisingly enough, the latter has received much less attention from the community. In this work, we aim at contributing to the advancement of process mining on uncertain data, considering in particular the problem of conformance checking \cite{CDSW18}. Specifically, our contribution is twofold:
\begin{compactenum}
\item We introduce a framework for data-aware conformance checking over uncertain logs, through a suitably extended notion of alignment. The framework employs Data Petri nets \cite{Mannhardt18} for reference process models, and addresses event logs incorporating sophisticated forms of uncertainty, pertaining the recorded timestamps, data values, and/or events. Notably, the framework comes with a generic cost function whose components can be flexibly instantiated to homogeneously account for a variety of conformance checking artefacts.
\item We devise a corresponding operational counterpart to effectively attack the problem of computing alignments and their costs. Instead of relying on ad-hoc algorithmic techniques, our approach builds on and extends \cite{cocomot} to encode the problem into the well-established automated reasoning framework of SMT. This allows us to employ state-of-the-art SMT solvers. 
\end{compactenum}

%
To handle uncertainty in the log, we follow the approach in~\cite{PegoraroUA21}, where the log is explicitly enriched with annotations reflecting the degree and nature of uncertainty. Such annotations may be derived from operational characteristics of the information system recording the event data (considering its logging precision and reliability), and/or by directly attaching them to the generated events. For instance, the log may be enriched by explicit details on the coarseness or precision of an automatic logging device (such as a sensor); alternatively, uncertainty-related annotations may be derived from domain knowledge on the precision and frequency of a specific human activity.

More specifically, our framework accounts for four main types of uncertain event data.
%
\begin{inparaenum}[(1)]
\item \emph{Uncertain events}: these are recorded in a log trace but come with a known \emph{confidence value}, capturing the degree of (un)certainty about the fact that a recorded event actually happened at all during the process execution.  %In the literature, these are also called indeterminate events;
\item \emph{Uncertain timestamps}: due to coarseness of the logging activity, events are in general not totally ordered, but come with a fixed range of possible timestamp values. This calls for considering multiple possible orderings:  a log trace is \emph{a set} of events rather than a sequence.
\item \emph{Uncertain activities}: this pertains events whose reference activity is not certainly known. Hence, the event comes with a candidate set of possible activities (each with its own confidence value). %This can be naturally extended to further event attributes beyond activity labels, although in this paper we focus on these;
\item \emph{Uncertain data values}: in the execution of data-aware processes, for instance due to sensor precision, event data attributes may come with both coarseness and ambiguity. Specifically, the log may only record a set of possible values or an interval for a given attribute, requiring all possible values to be considered. % for the conformance checking task. 
\end{inparaenum} 
%
It is important to stress that the notion of confidence used here should not be confused with that of probability. In fact, it measures the degree of trust in the recorded behaviour, which has nothing to do with the likelihood/frequency of such a behaviour.  %Notably, this allows us to explicitly single apart the notion of uncertain data from that of infrequent data.  

To account for these different types of uncertain event data, we borrow and adapt to our data-aware setting the notion of \emph{realization} from \cite{PegoraroUA21}. A realization of a log trace with uncertainty is an \emph{ordered sequence} of events in which the uncertainty of all types of event data above is resolved. Our task then concretely substantiated as follows: given a Data Petri net and a log trace  with uncertainty, find some realization of that trace that admits an \emph{optimal alignment}, i.e., an alignment of minimal cost among all possible realizations for that log trace. Differently from from \cite{PegoraroUA21}, the confidence values of the original trace are used as an integral part for measuring the cost incurred in selecting different realizations. 

Crucially, since we are in a data-aware setting, a log trace may correspond to infinitely many possible realizations. This is handled symbolically thanks to our SMT-based approach.


==> 6-experimental.tex <==
%!TEX root = main.tex

\section{Experimental}
\label{sec:experimental}

We implemented our conformance checking approach in
\tool, a proof-of-concept implementation based on the encoding in Sec. \ref{sec:encoding}.
Both tasks described in Sec.~\ref{sec:tasks} can be solved.
The source code is publicly available.\footnote{\url{https://github.com/bytekid/cocomot}}

The tool \tool is a Python command line script:
it takes as input a DPN (as \texttt{.pnml} file) and a log (as \texttt{.xes}) using the language extension describe in~\cite{Pegoraro21}.
The command line option \texttt{-u} triggers the use of the uncertainty module.
It then computes either a best-case realization (with parameter $\texttt{-u min}$),
or the expected fitness (with parameter $\texttt{-u fit}$).

% Experimental setup questions:
% \begin{itemize}
% \item do we consider logs with probabilities already as input?
% \item do we discuss preprocessing of non-probabilistic logs a la Pegoraro (i.e., logs with his uncertainty marks or with partially assigned probabilities) here?
% \end{itemize}


